Guaranteed Parameter Estimation for Discrete Energy Minimization

Structural learning, a method to estimate the parameters for discrete energy minimization, has been proven to be effective in solving computer vision problems, especially in 3D scene parsing. As the complexity of the models increases, structural learning algorithms turn to approximate inference to retain tractability. Unfortunately, such methods often fail because the approximation can be arbitrarily poor. In this work, we propose a method to overcome this limitation through exploiting the properties of the joint problem of training time inference and learning. With the help of the learning framework, we transform the inapproximable inference problem into a polynomial time solvable one, thereby enabling tractable exact inference while still allowing an arbitrary graph structure and full potential interactions. Our learning algorithm is guaranteed to return a solution with a bounded error to the global optimal within the feasible parameter space. We demonstrate the effectiveness of this method on two point cloud scene parsing datasets. Our approach runs much faster and solves a problem that is intractable for previous, well-known approaches.

==> Removed.tex <==
\begin{figure}[]
\begin{center}
   \includegraphics[width=0.7\linewidth]{figure/bridge.png}
\end{center}
   \caption{The synthetic bridge dataset. It is a large point dataset we constructed for large building structure scene understanding and recognition. Note besides the 7 class labels listed here, we have 4 additional less common labels. The labels are chosen according to domain specific knowledge.}
\label{fig:bridge}
\end{figure}

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.8\linewidth]{figure/snake.png}
% \end{center}
%   \caption{The Snake Dataset.}
% \label{fig:snake}
% \end{figure}

% \subsection{Snake Dataset: Ideal Case Intepretation}

% The snake dataset is constructed by \cite{nowozin2011decision} to test their contextual classification algorithm, Decision Tree Field (DTF). The 'snake' is a sequence of pixels adjacent to each other \ref{fig:snake}. The input is pixel colors encoding the direction of the next pixel. The label of a pixel is the index from the head, with head being 1.

% We first analyze what we should do for a non-structural classifier given these features:
% \begin{itemize}
% \item Local feature: This is impossible as we cannot learn a function that maps 4 elements to n elements. With n being the length of the snake.
% \item Contextual feature: in order to classify correctly, the neighborhood size needs to be very large. It is also challenging for the learning part as the configuration space is exponential.
% \end{itemize}

% In contrast, a structural classifier makes use of pairwise or higher order interactions and predict the labels jointly. In our experiment, we model each pixel as a node and use the 4 colors as unary features. We add a directed edge between the nodes according to the direction encoding in the color.







% For a non-structural classifier, we can constru


% MSR-snake, local feature does not make sense

% What 

% Have to predict nodes jointly.

% A structural classifier:

% Pairwise relationship can propagate in the graph

% Able to capture the inherent relationship

% % \begin{table}[t]
% % \renewcommand{\arraystretch}{1.05}
% % \centering
% % \footnotesize
% % \begin{tabular}{l|c|c|c}
% % \hline
% % Method \& dataset	    &GTEA(71)	    &Gaze(40)     &Gaze+(44)\\
% % \hline
% % Fathi \textit{et al.}\ \cite{fathi2011learning}  & 61.36    & N/A  & N/A\\
% % \hline
% % Motion CNN              & 67.74             & 38.05          & 61.87\\
% % \hline
% % Joint training          & 76.15          & 55.55          & 74.34\\
% % \hline
% % \end{tabular}
% % \vspace{-2mm}
% % \caption{{Average object recognition accuracy.} Our proposed method performs about 15\% better than \cite{fathi2011learning}. Joint training of motion and object networks constantly improves accuracy on all datasets.}
% % \label{tab-obj-results}
% % \vspace{-2mm}
% % \end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{l|lll}
% \hline
%          & DTF  & MRF  & Ours         \\ \hline
% Accuracy & 99.4 & 91.9 & \textbf{100} \\ \hline
% \end{tabular}
% }
% \vspace{4mm}
% \caption{Test Set Accuracy for the Snake Dataset. The results of the first two columns are from \cite{nowozin2011decision}}
% \label{tab:snake}
% \end{table}

% \begin{figure}[t]
% \begin{center}
%   \includegraphics[width=0.8\linewidth]{figure/snake2.png}
% \end{center}
%   \caption{Learned Potentials on the Snake Dataset.}
% \label{fig:snake2}
% \end{figure}


% \begin{table*}[t!] 
%   \begin{center}
%   \small
%   \begin{tabularx}{\textwidth}{| c | X | X | X | X | X | X | X | X | X | X | X |}
%     \hline
%      & M 11 & M 12 & M 13 & M 14 & M 16 & M 19 & M 22 & M 26 & M 27 & M 30 & Average\\ \hline
%     Axis error (deg) & 0.074 & 0.885 & 0.100 & 0.186 & 0.059 & 0.104 & 0.042 & 0.043 & 0.123 & 0.054 & 0.412 \\ \hline
%     Endpoint error (m) & 0.143 & 0.068 & 0.183 & 0.211 & 0.114 & 0.041 & 0.108 & 0.131 & 0.045 & 0.088 & 0.111 \\ \hline
%   \end{tabularx}
%   \end{center}
%   \caption{Quantitative evaluation of our method on the synthetic data. The averages are computed over all beams in all ten models.} \label{table}
% \end{table*}


% \begin{table}[]
% \centering
% \begin{tabular}{l|lll}
% \hline
%          & DTF  & MRF  & Ours         \\ \hline
% Accuracy & 99.4 & 91.9 & \textbf{100} \\ \hline
% \end{tabular}
% }
% \vspace{4mm}
% \caption{Test Set Accuracy for the Snake Dataset. The results of the first two columns are from \cite{nowozin2011decision}}
% \label{tab:snake}
% \end{table}
